Unveiling IPv6 Scanning Dynamics: A Longitudinal Study Using Large Scale Proactive and Passive IPv6 Telescopes

We introduce new tools and vantage points to develop and integrate proactive techniques to attract IPv6 scan traffic, thus enabling its analysis. By deploying the largest-ever IPv6 proactive telescope in a production ISP network, we collected over 600M packets of unsolicited traffic from 1.9k Autonomous Systems in 10 months. We characterized the sources of unsolicited traffic, evaluated the effectiveness of five major features across the network stack, and inferred scanners' sources of target addresses and their strategies.

==> Makefile <==
# Makefile for LaTeX files
# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile
# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.
# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo
# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 
# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 
# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $
LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
DATE=$(shell date +%Y-%m-%d)
COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false
# These are OK
SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)
# These are not
#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))
define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef
define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef
define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef
define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef
define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef
define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef
all 	: $(TRG)
.PHONY	: all show clean ps pdf showps veryclean
clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)
veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~
# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 
include $(SRC:.tex=.d)
# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)
$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@
#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)
show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done
showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done
ps	: $(PSF) 
pdf	: $(PDF) 
# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)
######################################################################
# Define rules for EPS source files.
# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12
#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))

==> draft.tex <==
Hosts on the internet are persistently targeted by malicious actors in an attempt to compromise financial assets and/or sensitive personal records. To achieve this, malicious actors make use of internet scanning to identify potentially vulnerable services and consequently exploit them. On the other hand, researchers and security organizations develop methodologies and tools to understand scanner behaviors and thwart scanning campaigns.

The internet scanning ecosystem has largely been studied in the context of the IPv4 address space. This has been enabled by the 


==> tables/telescope_summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[tbh]
% \label{tab:telescope_summary}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|cccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Telescope}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Address \\ space\end{tabular}}} & \multirow{2}{*}{\textbf{Location}}                       & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Network \\ type\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Measurement\\ start date\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Unsolicited packets \\ received\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Unique traffic sources}}                                                                      & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unique destinations \\ targeted\end{tabular}}}      \\ \cline{7-13} 
                                    &                                                                                    &                                                          &                                                                                   &                                                                                            &                                                                                                   & \multicolumn{1}{c|}{\textbf{/128}} & \multicolumn{1}{c|}{\textbf{/64}} & \multicolumn{1}{c|}{\textbf{/48}} & \textbf{ASN} & \multicolumn{1}{c|}{\textbf{/128}} & \multicolumn{1}{l|}{\textbf{/64}} & \multicolumn{1}{l|}{\textbf{/48}} \\ \hline
\textit{\textbf{NT-A}}              & /32                                                                                & \begin{tabular}[c]{@{}c@{}}Southern \\ Asia\end{tabular} & \begin{tabular}[c]{@{}c@{}}Transit \\ ISP\end{tabular}                            & 07/23                                                                                      & 654M                                                                                              & \multicolumn{1}{c|}{259k}          & \multicolumn{1}{c|}{190k}         & \multicolumn{1}{c|}{138k}         & 1.9k         & \multicolumn{1}{c|}{134M}          & \multicolumn{1}{c|}{3.1M}         & 61.5k                             \\ \hline
\textit{\textbf{NT-B}}              & /48                                                                                & Ireland                                                  & Research                                                                          & 01/23                                                                                      & 300k                                                                                              & \multicolumn{1}{c|}{1.9k}          & \multicolumn{1}{c|}{367}          & \multicolumn{1}{c|}{354}          & 60           & \multicolumn{1}{c|}{100k}          & \multicolumn{1}{c|}{65.5k}        & 1                                 \\ \hline
\textit{\textbf{NT-C}}              & /32                                                                                & \begin{tabular}[c]{@{}c@{}}United \\ States\end{tabular} & Academic                                                                          & 10/23                                                                                      & 250M                                                                                              & \multicolumn{1}{c|}{57k}           & \multicolumn{1}{c|}{26k}          & \multicolumn{1}{c|}{24k}          & 507          & \multicolumn{1}{c|}{21M}           & \multicolumn{1}{c|}{14.9M}        & 48.8k                             \\ \hline
\end{tabular}%
}
\end{table*}
